A Critical Evaluation of Evaluations for Long-form Question Answering

Long-form question answering (LFQA) enables answering a wide range of questions, but its flexibility poses enormous challenges for evaluation. We perform the first targeted study of the evaluation of long-form answers, covering both human and automatic evaluation practices. We hire domain experts in seven areas to provide preference judgments over pairs of answers, along with free-form justifications for their choices. We present a careful analysis of experts' evaluation, which focuses on new aspects such as the comprehensiveness of the answer. Next, we examine automatic text generation metrics, finding that no existing metrics are predictive of human preference judgments. However, some metrics correlate with fine-grained aspects of answers (e.g., coherence). We encourage future work to move away from a single "overall score" of the answer and adopt a multi-faceted evaluation, targeting aspects such as factuality and completeness. We publicly release all of our annotations and code to spur future work into LFQA evaluation.

==> figs/_comment_analysis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{figure*}
\begin{tikzpicture}[
/pgfplots/every axis/.style={
  width=\textwidth,
  height=.31\textwidth,
  font=\footnotesize,}]

\definecolor{burlywood239183145}{RGB}{239,183,145}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsteelblue171201233}{RGB}{171,201,233}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={},
xmin=-0.5, xmax=13.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13},
xticklabel style={rotate=15.0, font=\tiny},
xticklabels={
  Supported,
  Coherence,
  Relevance,
  Conciseness,
  Easy to follow,
  Detailed,
  Informative,
  Completeness,
  Well formulated,
  Grammar,
  Example,
  Factuality,
  Clearness,
  Depth,
},
y grid style={darkgray176},
ylabel={count},
ymin=0, ymax=36,
ytick style={color=black},
yticklabel style={font=\tiny},
]
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:-0.4,0) rectangle (axis cs:0,33);
\addlegendimage{ybar,ybar legend,draw=none,fill=lightsteelblue171201233}
\addlegendentry{webgpt}

\draw[draw=none,fill=lightsteelblue171201233] (axis cs:0.6,0) rectangle (axis cs:1,29);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:1.6,0) rectangle (axis cs:2,27);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:2.6,0) rectangle (axis cs:3,24);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:3.6,0) rectangle (axis cs:4,15);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:4.6,0) rectangle (axis cs:5,14);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:5.6,0) rectangle (axis cs:6,13);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:6.6,0) rectangle (axis cs:7,13);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:7.6,0) rectangle (axis cs:8,4);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:8.6,0) rectangle (axis cs:9,4);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:9.6,0) rectangle (axis cs:10,1);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:10.6,0) rectangle (axis cs:11,0);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:11.6,0) rectangle (axis cs:12,0);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:12.6,0) rectangle (axis cs:13,0);
\draw[draw=none,fill=burlywood239183145] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=burlywood239183145}
\addlegendentry{expert}

\draw[draw=none,fill=burlywood239183145] (axis cs:1,0) rectangle (axis cs:1.4,0);
\draw[draw=none,fill=burlywood239183145] (axis cs:2,0) rectangle (axis cs:2.4,31);
\draw[draw=none,fill=burlywood239183145] (axis cs:3,0) rectangle (axis cs:3.4,0);
\draw[draw=none,fill=burlywood239183145] (axis cs:4,0) rectangle (axis cs:4.4,21);
\draw[draw=none,fill=burlywood239183145] (axis cs:5,0) rectangle (axis cs:5.4,10);
\draw[draw=none,fill=burlywood239183145] (axis cs:6,0) rectangle (axis cs:6.4,0);
\draw[draw=none,fill=burlywood239183145] (axis cs:7,0) rectangle (axis cs:7.4,29);
\draw[draw=none,fill=burlywood239183145] (axis cs:8,0) rectangle (axis cs:8.4,17);
\draw[draw=none,fill=burlywood239183145] (axis cs:9,0) rectangle (axis cs:9.4,17);
\draw[draw=none,fill=burlywood239183145] (axis cs:10,0) rectangle (axis cs:10.4,13);
\draw[draw=none,fill=burlywood239183145] (axis cs:11,0) rectangle (axis cs:11.4,29);
\draw[draw=none,fill=burlywood239183145] (axis cs:12,0) rectangle (axis cs:12.4,10);
\draw[draw=none,fill=burlywood239183145] (axis cs:13,0) rectangle (axis cs:13.4,2);
\draw[draw=none,fill=steelblue49115161] (axis cs:-0.4,0) rectangle (axis cs:0,24);
\draw[draw=none,fill=steelblue49115161] (axis cs:0.6,0) rectangle (axis cs:1,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:1.6,0) rectangle (axis cs:2,14);
\draw[draw=none,fill=steelblue49115161] (axis cs:2.6,0) rectangle (axis cs:3,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:3.6,0) rectangle (axis cs:4,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:4.6,0) rectangle (axis cs:5,9);
\draw[draw=none,fill=steelblue49115161] (axis cs:5.6,0) rectangle (axis cs:6,10);
\draw[draw=none,fill=steelblue49115161] (axis cs:6.6,0) rectangle (axis cs:7,9);
\draw[draw=none,fill=steelblue49115161] (axis cs:7.6,0) rectangle (axis cs:8,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:8.6,0) rectangle (axis cs:9,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:9.6,0) rectangle (axis cs:10,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:10.6,0) rectangle (axis cs:11,0);
\draw[draw=none,fill=steelblue49115161] (axis cs:11.6,0) rectangle (axis cs:12,0);
\draw[draw=none,fill=steelblue49115161] (axis cs:12.6,0) rectangle (axis cs:13,0);
\draw[draw=none,fill=peru22412844] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=peru22412844] (axis cs:1,0) rectangle (axis cs:1.4,0);
\draw[draw=none,fill=peru22412844] (axis cs:2,0) rectangle (axis cs:2.4,11);
\draw[draw=none,fill=peru22412844] (axis cs:3,0) rectangle (axis cs:3.4,0);
\draw[draw=none,fill=peru22412844] (axis cs:4,0) rectangle (axis cs:4.4,12);
\draw[draw=none,fill=peru22412844] (axis cs:5,0) rectangle (axis cs:5.4,8);
\draw[draw=none,fill=peru22412844] (axis cs:6,0) rectangle (axis cs:6.4,0);
\draw[draw=none,fill=peru22412844] (axis cs:7,0) rectangle (axis cs:7.4,20);
\draw[draw=none,fill=peru22412844] (axis cs:8,0) rectangle (axis cs:8.4,10);
\draw[draw=none,fill=peru22412844] (axis cs:9,0) rectangle (axis cs:9.4,1);
\draw[draw=none,fill=peru22412844] (axis cs:10,0) rectangle (axis cs:10.4,9);
\draw[draw=none,fill=peru22412844] (axis cs:11,0) rectangle (axis cs:11.4,15);
\draw[draw=none,fill=peru22412844] (axis cs:12,0) rectangle (axis cs:12.4,6);
\draw[draw=none,fill=peru22412844] (axis cs:13,0) rectangle (axis cs:13.4,2);
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
-0.2 0
-0.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.8 0
0.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.8 0
1.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.8 0
2.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.8 0
3.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.8 0
4.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.8 0
5.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.8 0
6.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.8 0
7.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.8 0
8.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.8 0
9.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.8 0
10.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.8 0
11.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.8 0
12.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.2 0
0.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.2 0
1.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.2 0
2.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.2 0
3.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.2 0
4.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.2 0
5.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.2 0
6.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.2 0
7.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.2 0
8.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.2 0
9.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.2 0
10.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.2 0
11.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.2 0
12.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
13.2 0
13.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
-0.2 0
-0.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.8 0
0.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.8 0
1.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.8 0
2.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.8 0
3.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.8 0
4.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.8 0
5.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.8 0
6.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.8 0
7.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.8 0
8.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.8 0
9.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.8 0
10.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.8 0
11.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.8 0
12.8 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.2 0
0.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.2 0
1.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.2 0
2.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.2 0
3.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.2 0
4.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.2 0
5.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.2 0
6.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.2 0
7.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.2 0
8.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.2 0
9.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.2 0
10.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.2 0
11.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.2 0
12.2 0
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
13.2 0
13.2 0
};

%depth
\draw (axis cs:13.2,1.5) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 2};

% clearness 
\draw (axis cs:12.2,6) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 6};

\draw (axis cs:12.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

% factuality
\draw (axis cs:11.2,15) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 15};

\draw (axis cs:11.2,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};

% example 
\draw (axis cs:10.2,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};


\draw (axis cs:10.2,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:9.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% grammar
\draw (axis cs:9.2,17) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 17};

\draw (axis cs:9.2,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

\draw (axis cs:8.8,4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 4};

\draw (axis cs:8.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% well formulated 
\draw (axis cs:8.2,17) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 17};

\draw (axis cs:8.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};


\draw (axis cs:7.8,4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 4};

\draw (axis cs:7.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% completeness

\draw (axis cs:7.2,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};

\draw (axis cs:7.2,20) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 20};

\draw (axis cs:6.8,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:6.8,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};

% informative
\draw (axis cs:5.8,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:5.8,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

% detail 

\draw (axis cs:5.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

\draw (axis cs:5.2,7.4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 8};

\draw (axis cs:4.8,14) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 14};

\draw (axis cs:4.8,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};

% easy to follow
\draw (axis cs:4.2,21) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 21};

\draw (axis cs:4.2,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

\draw (axis cs:3.8,15) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 15};

\draw (axis cs:3.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

% conciseness
\draw (axis cs:2.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

\draw (axis cs:2.8,24) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 24};

% relevance

\draw (axis cs:2.2,31) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 31};

\draw (axis cs:2.2,11) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 11};

\draw (axis cs:1.8,27) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 27};

\draw (axis cs:1.8,14) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 14};

% coherence 
\draw (axis cs:0.8,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};

\draw (axis cs:0.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

% supported 
\draw (axis cs:-0.2,33) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 33};

\draw (axis cs:-0.2,24) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 24};
\end{axis}

\end{tikzpicture}
\caption{By manual analysis of 52 comments written by experts and 60 WebGPT comments, we find 14 aspects that are frequently mentioned. We count the occurrence of each aspect (the lighter bar) and how many times each aspect was a decisive aspect (the darker bar) for the annotators to make their decision.}\vspace{-0.25em}
\label{fig:manual_comment_analysis}
\end{figure*}


==> figs/comment_analysis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{figure*}
\begin{tikzpicture}[
/pgfplots/every axis/.style={
  width=\textwidth,
  height=.31\textwidth,
  font=\footnotesize,}]

\definecolor{burlywood239183145}{RGB}{239,183,145}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightsteelblue171201233}{RGB}{171,201,233}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xlabel={},
xmin=-0.5, xmax=12.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
xticklabel style={rotate=15.0, font=\tiny},
xticklabels={
  Factuality,
  Coherence,
  Relevance,
  Conciseness,
  Easy to follow,
  Detail,
  Informative,
  Completeness,
  Well formulated,
  Grammar,
  Example,
  Clearness,
  Depth
},
y grid style={darkgray176},
ylabel={count},
ymin=0, ymax=36,
ytick style={color=black},
yticklabel style={font=\tiny},
]
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:-0.4,0) rectangle (axis cs:0,33);
\addlegendimage{ybar,ybar legend,draw=none,fill=lightsteelblue171201233}
\addlegendentry{webgpt}

\draw[draw=none,fill=lightsteelblue171201233] (axis cs:0.6,0) rectangle (axis cs:1,29);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:1.6,0) rectangle (axis cs:2,27);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:2.6,0) rectangle (axis cs:3,24);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:3.6,0) rectangle (axis cs:4,15);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:4.6,0) rectangle (axis cs:5,14);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:5.6,0) rectangle (axis cs:6,13);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:6.6,0) rectangle (axis cs:7,13);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:7.6,0) rectangle (axis cs:8,4);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:8.6,0) rectangle (axis cs:9,4);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:9.6,0) rectangle (axis cs:10,1);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:10.6,0) rectangle (axis cs:11,nan);
\draw[draw=none,fill=lightsteelblue171201233] (axis cs:11.6,0) rectangle (axis cs:12,nan);
\draw[draw=none,fill=burlywood239183145] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,29);
\addlegendimage{ybar,ybar legend,draw=none,fill=burlywood239183145}
\addlegendentry{expert}

\draw[draw=none,fill=burlywood239183145] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=burlywood239183145] (axis cs:2,0) rectangle (axis cs:2.4,31);
\draw[draw=none,fill=burlywood239183145] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=burlywood239183145] (axis cs:4,0) rectangle (axis cs:4.4,21);
\draw[draw=none,fill=burlywood239183145] (axis cs:5,0) rectangle (axis cs:5.4,10);
\draw[draw=none,fill=burlywood239183145] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=burlywood239183145] (axis cs:7,0) rectangle (axis cs:7.4,29);
\draw[draw=none,fill=burlywood239183145] (axis cs:8,0) rectangle (axis cs:8.4,17);
\draw[draw=none,fill=burlywood239183145] (axis cs:9,0) rectangle (axis cs:9.4,17);
\draw[draw=none,fill=burlywood239183145] (axis cs:10,0) rectangle (axis cs:10.4,13);
\draw[draw=none,fill=burlywood239183145] (axis cs:11,0) rectangle (axis cs:11.4,10);
\draw[draw=none,fill=burlywood239183145] (axis cs:12,0) rectangle (axis cs:12.4,2);
\draw[draw=none,fill=steelblue49115161] (axis cs:-0.4,0) rectangle (axis cs:0,24);
\draw[draw=none,fill=steelblue49115161] (axis cs:0.6,0) rectangle (axis cs:1,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:1.6,0) rectangle (axis cs:2,14);
\draw[draw=none,fill=steelblue49115161] (axis cs:2.6,0) rectangle (axis cs:3,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:3.6,0) rectangle (axis cs:4,12);
\draw[draw=none,fill=steelblue49115161] (axis cs:4.6,0) rectangle (axis cs:5,9);
\draw[draw=none,fill=steelblue49115161] (axis cs:5.6,0) rectangle (axis cs:6,10);
\draw[draw=none,fill=steelblue49115161] (axis cs:6.6,0) rectangle (axis cs:7,9);
\draw[draw=none,fill=steelblue49115161] (axis cs:7.6,0) rectangle (axis cs:8,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:8.6,0) rectangle (axis cs:9,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:9.6,0) rectangle (axis cs:10,1);
\draw[draw=none,fill=steelblue49115161] (axis cs:10.6,0) rectangle (axis cs:11,nan);
\draw[draw=none,fill=steelblue49115161] (axis cs:11.6,0) rectangle (axis cs:12,nan);
\draw[draw=none,fill=peru22412844] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,15);
\draw[draw=none,fill=peru22412844] (axis cs:1,0) rectangle (axis cs:1.4,nan);
\draw[draw=none,fill=peru22412844] (axis cs:2,0) rectangle (axis cs:2.4,11);
\draw[draw=none,fill=peru22412844] (axis cs:3,0) rectangle (axis cs:3.4,nan);
\draw[draw=none,fill=peru22412844] (axis cs:4,0) rectangle (axis cs:4.4,12);
\draw[draw=none,fill=peru22412844] (axis cs:5,0) rectangle (axis cs:5.4,8);
\draw[draw=none,fill=peru22412844] (axis cs:6,0) rectangle (axis cs:6.4,nan);
\draw[draw=none,fill=peru22412844] (axis cs:7,0) rectangle (axis cs:7.4,20);
\draw[draw=none,fill=peru22412844] (axis cs:8,0) rectangle (axis cs:8.4,10);
\draw[draw=none,fill=peru22412844] (axis cs:9,0) rectangle (axis cs:9.4,1);
\draw[draw=none,fill=peru22412844] (axis cs:10,0) rectangle (axis cs:10.4,9);
\draw[draw=none,fill=peru22412844] (axis cs:11,0) rectangle (axis cs:11.4,6);
\draw[draw=none,fill=peru22412844] (axis cs:12,0) rectangle (axis cs:12.4,2);
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.8 nan
2.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.8 nan
3.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.8 nan
4.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.8 nan
5.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.8 nan
6.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.8 nan
7.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.8 nan
8.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.8 nan
9.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.8 nan
10.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.8 nan
11.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.2 nan
2.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.2 nan
3.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.2 nan
4.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.2 nan
5.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.2 nan
6.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.2 nan
7.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.2 nan
8.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.2 nan
9.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.2 nan
10.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.2 nan
11.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.2 nan
12.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.8 nan
2.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.8 nan
3.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.8 nan
4.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.8 nan
5.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.8 nan
6.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.8 nan
7.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.8 nan
8.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.8 nan
9.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.8 nan
10.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.8 nan
11.8 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
2.2 nan
2.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
3.2 nan
3.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
4.2 nan
4.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
5.2 nan
5.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
6.2 nan
6.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
7.2 nan
7.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
8.2 nan
8.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
9.2 nan
9.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
10.2 nan
10.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
11.2 nan
11.2 nan
};
\addplot [line width=1.08pt, darkslategray66, forget plot]
table {%
12.2 nan
12.2 nan
};

%depth
\draw (axis cs:12.2,1.5) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 2};

% clearness 
\draw (axis cs:11.2,6) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 6};

\draw (axis cs:11.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

% example 
\draw (axis cs:10.2,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};


\draw (axis cs:10.2,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:9.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% grammar
\draw (axis cs:9.2,17) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 17};

\draw (axis cs:9.2,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

\draw (axis cs:8.8,4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 4};

\draw (axis cs:8.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% well formulated 
\draw (axis cs:8.2,17) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 17};

\draw (axis cs:8.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};


\draw (axis cs:7.8,4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 4};

\draw (axis cs:7.8,1) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 1};

% completeness

\draw (axis cs:7.2,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};

\draw (axis cs:7.2,20) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 20};

\draw (axis cs:6.8,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:6.8,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};

% informative
\draw (axis cs:5.8,13) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 13};

\draw (axis cs:5.8,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

% detail 

\draw (axis cs:5.2,10) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 10};

\draw (axis cs:5.2,7.4) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 8};

\draw (axis cs:4.8,14) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 14};

\draw (axis cs:4.8,9) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 9};

% easy to follow
\draw (axis cs:4.2,21) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 21};

\draw (axis cs:4.2,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

\draw (axis cs:3.8,15) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 15};

\draw (axis cs:3.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

% conciseness
\draw (axis cs:2.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

\draw (axis cs:2.8,24) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 24};

% relevance

\draw (axis cs:2.2,31) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 31};

\draw (axis cs:2.2,11) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 11};

\draw (axis cs:1.8,27) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 27};

\draw (axis cs:1.8,14) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 14};

% coherence 
\draw (axis cs:0.8,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};

\draw (axis cs:0.8,12) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 12};

% supported 
\draw (axis cs:-0.2,33) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 33};

\draw (axis cs:-0.2,24) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 24};

% factuality
\draw (axis cs:0.2,15) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 15};

\draw (axis cs:0.2,29) node[
  scale=0.5,
  anchor=south,
  text=black,
  rotate=0.0
]{\large 29};



\end{axis}

\end{tikzpicture}
\caption{By manual analysis of 52 comments written by experts and 60 WebGPT comments, we find 13 aspects that are frequently mentioned. We plot the occurrence of each aspect (the lighter bar) and how many times each aspect was a decisive aspect (the darker bar) for the annotators to make their decision. Examples of annotator explanations and extracted aspects are in the Table \ref{tab:explanation_example}. \fy{to be updated}}\vspace{-0.25em}
\label{fig:manual_comment_analysis}
\end{figure*}


==> table_1.tex <==
\begin{table*}[ht]
\small
\begin{center}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Metrics} &\textbf{Acc(W-h/m)} & \textbf{Acc(W-m/m)} & \textbf{Acc(H-h/m)} & \textbf{Acc(H-m/m)} & \textbf{Expert}\\
\midrule
\multicolumn{6}{c}{\textit{\textbf{Overall comparison}}}\vspace{0.1cm}\\
\# pairs of data & 637 & 1,923 & 419 & 370 & 140 \\
ROUGE & 0.53 & 0.53 & 0.43 & 0.52 &  -\\
BERTScore & 0.57 & 0.51 & 0.45 & \textbf{0.61} &  -\\
%BLEURT & 0.52 &  0.54 &  &   &  -\\
Self-bleu & 0.50 & 0.45 & 0.57 & 0.48 & 0.36\\
PPL & 0.48 &  0.51 & 0.28 & 0.52 & 0.61\\
Length & 0.52 & \textbf{0.57} & 0.61 & 0.48 & \textbf{0.69} \\
QG likelihood & \textbf{0.58} & 0.51 & 0.61 & 0.60 & 0.61\\
RankGen & \textbf{0.58} & 0.52  & \textbf{0.63} & 0.54 & 0.59\\ 
BARTScore & 0.57 & 0.49  & 0.58 & 0.55 & \\ 
QA\_eval\_lerc & 0.50 &  0.54 & - & - &  - \\
\midrule
longformer(Q, A) &  \textbf{0.62} &  0.59 &  0.60 & \textbf{0.62} & \textbf{0.69} \\
longformer(Q, A, D) &  0.60 &  \textbf{0.60} & - & - & - \\
175B reward model* & - & 0.65-0.70 & - & - & - \\
Human* & - & 0.70-0.75 & - & - & - \\
\midrule
\multicolumn{6}{c}{\textit{\textbf{Coherence comparison}}}\vspace{0.1cm}\\
\# pairs of data & 496 & - & 164 & 194 &  \\
ROUGE & 0.54 & - & 0.46 & 0.48 &  \\
BERTScore & \textbf{0.62} & - & 0.39 & \textbf{0.69} & \\
%BLEURT & 0.52 &  &  &   &  -\\
Self-bleu & 0.59& - & 0.64 & 0.61 \\ 
PPL & 0.46 & - & 0.21  & 0.34 \\
Length & 0.39 & - & 0.62  & 0.49 \\
QG likelihood & 0.56 & - & 0.59 & 0.50 \\ 
RankGen & 0.59 & - & \textbf{0.66} & 0.55 \\ 
BARTScore & 0.55 & -  & 0.55 & 0.48& \\ 
QA\_eval\_lerc & 0.48 & - & - & - & \\
%roberta(Q, A) & 0.48 & - & 0.64 & 0.65 \\
%roberta(Q, A, D) & 0.49 &  - & - & - \\
\midrule
longformer(Q, A) & 0.56 & - & 0.62 & 0.65 \\
longformer(Q, A, D) & 0.54 &  - & - & - \\
\midrule
\multicolumn{6}{c}{\textit{\textbf{Factuality comparison}}}\vspace{0.1cm}\\
\# pairs of data & 149 & - & 151 & 169 &  \\
ROUGE & 0.46 & - & 0.40 & 0.51 & \\
BERTScore & 0.48 & - & 0.39 & 0.61 & \\
%BLEURT & 0.46 &  &  &   &  -\\
Self-bleu & 0.49 & - & 0.62 & 0.47 &  \\ 
PPL & 0.47 & - & 0.19 & 0.44 & \\
Length & 0.57 & - & \textbf{0.68} & 0.57 \\ 
QG likelihood & 0.56 & - & 0.64 & 0.48 & \\
RankGen & 0.58 & - & 0.66 & 0.53 & \\
BARTScore & 0.58 & -  &  0.58 & 0.53 & \\ 
QA\_eval\_lerc & \textbf{0.69} & - & - & - & \\
%roberta(Q, A) & 0.58 & - & 0.64 & 0.58 \\
%roberta(Q, A, D) & 0.62 &  - & - & - \\
\midrule
longformer(Q, A) & 0.63 & - & 0.63 & \textbf{0.63} \\
longformer(Q, A, D) & 0.65 &  - & - & - \\
\bottomrule
\end{tabular} 
\end{center}\vspace{-0.3em}
\caption{Ranking accuracy of different automatic metrics for comparisons of various evaluation aspects. W(h/m) denotes comparisons between WebGPT model-generated answers and human demonstrations while H(m/m) denotes comparisons between pairs of Hurdles model-generated answers. *These are numbers reported in the WebGPT \cite{nakano2021webgpt} paper, which are not evaluated on the same set of data. 
%\ec{maybe add a column showing whether metric is learned or not?}
}
\label{tab:overall_comparisons}
\end{table*}
